Relative gradient optimization of the Jacobian term in unsupervised deep learning

Learning expressive probabilistic models correctly describing the data is a ubiquitous problem in machine learning. A popular approach for solving it is mapping the observations into a representation space with a simple joint distribution, which can typically be written as a product of its marginals -- thus drawing a connection with the field of nonlinear independent component analysis. Deep density models have been widely used for this task, but their maximum likelihood based training requires estimating the log-determinant of the Jacobian and is computationally expensive, thus imposing a trade-off between computation and expressive power. In this work, we propose a new approach for exact training of such neural networks. Based on relative gradients, we exploit the matrix structure of neural network parameters to compute updates efficiently even in high-dimensional spaces; the computational cost of the training is quadratic in the input size, in contrast with the cubic scaling of naive approaches. This allows fast training with objective functions involving the log-determinant of the Jacobian, without imposing constraints on its structure, in stark contrast to autoregressive normalizing flows.

==> app/d_augmentation.tex <==
Let's consider our sources $s$ to be normally distributed and our data to be images. $\bm{x}$ denotes a single sample, $x_i$ a single pixel (a single dimension). The density of the trained model can be written as the density of the sum of single-pixel contributions:

\begin{align}
    p(\bm{s}) &= \prod p(s_i) \\
    p(s_i) &= p(g(\bm{x})) = p(\sum g(x_i)) = p(\sum w_i t_i)
\end{align}

where $w_i$ is the weight that the neural network $g$ learns for each pixel, and $t$ is the unweighted single-pixel contribution. We learn our model such that $p(\bm{s})$ is normal, thus the $t_i$ must be Gaussian (Cramer's theorem). If we assum the weights $w_i$ to be constant, it is then easy to compute the single-pixel density estimations $p(t_i)$.


==> app/figures.tex <==
\begin{figure}
    \centering
        \begin{minipage}{.32\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeuRIPS2020/figures/toy_density/original.png}
            % \caption{}
            \end{subfigure}
            \vfill
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeuRIPS2020/figures/toy_density/original.png}
            % \caption{}
            \end{subfigure}%    
            % \caption{Main caption}
        \end{minipage}
        \hfill
        \begin{minipage}{.32\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeuRIPS2020/figures/toy_density/original.png}
            % \caption{}
            \end{subfigure}
            \vfill
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeuRIPS2020/figures/toy_density/original.png}
            % \caption{}
            \end{subfigure}%    
            % \caption{Main caption}
        \end{minipage}
        \hfill
        \begin{minipage}{.32\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeuRIPS2020/figures/toy_density/original.png}
            % \caption{}
            \end{subfigure}
            \vfill
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeuRIPS2020/figures/toy_density/original.png}
            % \caption{}
            \end{subfigure}%    
            % \caption{Main caption}
        \end{minipage}%
        \caption{Lowest caption}
    \end{figure}

\clearpage

\begin{figure}
    \centering
    \begin{minipage}{.5\linewidth}
    \centering
    \subfloat[]{\label{main:a}
    \includegraphics[scale=0.35]{NeuRIPS2020/figures/corr_vs_nu.jpeg}
    }
    \end{minipage}%
    \begin{minipage}{.4\linewidth}
    \centering
    \subfloat[]{\label{main:b}
    \includegraphics[scale=0.5]{NeuRIPS2020/figures/mixture.png}
    }
    \end{minipage}%\par\medskip
    
    \caption{(a) MCC between true and reconstructed sources for a nonstationary, nonlinear ICA model, under different number of layers and time segments; (b) Density estimation in a toy mixture model.}
    \label{fig:loss_and_grads}
\end{figure}

\clearpage

\begin{figure}
\centering
\include{NeuRIPS2020/figures/trick_vs_notrick}
\caption{}
\label{}
\end{figure}
%
%\begin{figure}[t!]
%    \centering
%    \begin{minipage}{.5\linewidth}
%    \centering
%    \subfloat[]{\label{main:a}
%    \includegraphics[scale=0.45]{NeuRIPS2020/figures/rel_vs_ordinary/trick_vs_notrick.pdf}
%    }
%    \end{minipage}%
%    \begin{minipage}{.5\linewidth}
%    \centering
%    \subfloat[]{\label{main:b}
%    \includegraphics[scale=0.45]{NeuRIPS2020/figures/main.pdf}
%    }
%    \end{minipage}%\par\medskip
%    % \begin{minipage}{.3\linewidth}
%    % \centering
%    % \subfloat[]{\label{main:c}
%    % \includegraphics[scale=0.4]{NeuRIPS2020/figures/Grad_norms_1.png}
%    % }
%    % \end{minipage}
%    \caption{(a) Comparison of the computation times required for $100$ gradient evaluations in a $n$-layer Neural Network with dimensionality of the data $D$.; (b) Comparison between the descent dynamics induced by (...).}
%    \label{fig:loss_and_grads}
%\end{figure}

\clearpage

\begin{figure}[t!]
    \centering
    \begin{minipage}{.5\linewidth}
    \centering
    \subfloat[]{\label{main:a}
    \includegraphics[scale=0.4]{NeuRIPS2020/figures/complexity/comparison_gpu_loglog.png}
    }
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
    \centering
    \subfloat[]{\label{main:b}
    \includegraphics[scale=0.4]{NeuRIPS2020/figures/complexity/comparison_gpu_linlin.png}
    }
    \end{minipage}%\par\medskip
    % \begin{minipage}{.3\linewidth}
    % \centering
    % \subfloat[]{\label{main:c}
    % \includegraphics[scale=0.4]{NeuRIPS2020/figures/Grad_norms_1.png}
    % }
    % \end{minipage}
    \caption{(a) Comparison of the computation times required for $100$ gradient evaluations in a $n$-layer Neural Network with dimensionality of the data $D$.; (b) Comparison between the descent dynamics induced by (...).}
    \label{fig:loss_and_grads}
\end{figure}

\begin{figure}
\centering
\include{NeuRIPS2020/figures/e_10_feat_0.png}
\caption{}
\label{}
\end{figure}

\begin{figure}
\centering
\include{NeuRIPS2020/figures/e_10_feat_t_0.png}
\caption{}
\label{}
\end{figure}

\begin{figure}
\centering
\include{NeuRIPS2020/figures/10_gen.png}
\caption{}
\label{}
\end{figure}

==> app/nonlinearities.tex <==
In the following, we provide some details regarding the nonlinearities we employ
\luigi{Mention that both are relatively smooth can be inverted easily with a Newton method; in practice, for our parameter choice, we use a fixed number of $100$ iterations which seems to be (way) more than sufficient.}

==> sec/rel_work.tex <==
% % \paragraph{Natural and Relative Gradients}

% % \textbf{Normalizing flows}
% % The modern conception of normalizing flows was introduced in~\cite{tabak2013family}, which discussed density estimation through the composition of simple maps. In~\cite{rippel2013high}, it was then proposed that deep density models implemented through neural networks could be used in order to construct bijective maps to a representation space and obtain normalized probability density estimates. Since then, the focus mainly shifted to scalability; \cite{dinh2014nice, dinh2016density} introduced scalable architectures, further refined in~\cite{kingma2018glow} to make them more scalable and suitable for practical applications; ~\cite{rezende2015variational} applied the results to variational inference. 
% Comprehensive reviews on normalizing flows can be found in~\cite{papamakarios2019normalizing, kobyzev2019normalizing}. 

% \textbf{Autoregressive flows}
% Autoregressive flows are among the most used in practice. They involve maps which can be written as
% $\mathrm{z}_{i}^{\prime}=\tau\left(\mathrm{z}_{i} ; \boldsymbol{h}_{i}\right) \quad$~, with $\quad \boldsymbol{h}_{i}=c_{i}\left(\mathbf{z}_{<i}\right)$~; $\tau$ is termed the \emph{transformer} and is a strictly monotonic function of $\mathrm{z}_{i}$, and $c_i$ the $i$-th \emph{conditioner}. Its constraint is that the $i-$th conditioner can only take as input variables with dimension indices less than $i$. This results in an overall transformation with a triangular Jacobian; the determinant is therefore tractable and can be computed in $\mathcal{O}(D)$ time. Autoregressive flows differ in the way the transformer and conditioner are implemented; most commonly used are affine autoregressive flows \cite{dinh2014nice, dinh2016density, kingma2016improved, papamakarios2017masked, kingma2018glow} and non-affine neural transformers \cite{huang2018neural}.
% Notice that the model we optimize in this paper has elsewhere been termed \emph{linear} flow~\cite{papamakarios2019normalizing}; linear flows are a strict generalization of autoregressive flows. 

% % \textbf{Flows based on residual transformations}
% % Another class of normalizing flows is based on invertible transformations of the form $\mathbf{z}^{\prime}=\mathbf{z}+g_{\phi}(\mathbf{z})$; this kind of flows are termed \emph{residual flows}. Two main approaches can be applied to build invertible residual flows: the first exploits the matrix determinant lemma and also results in determinants with $\mathcal{O}(D)$ computation time; however, there is no analytical way of computing their inverse. Examples of these approaches are Sylvester flows~\cite{berg2018sylvester}, planar flows~\cite{rezende2015variational} and radial flows~\cite{tabak2013family,rezende2015variational}. The second is approach is that of contractive flows~\cite{behrmann2018invertible}: in this case, the determinant can not be computed simply; likelihood-based training of these models therefore needs to rely on a Hutchkinson's trace based approximation to the exact log-likelihood.

% Other related methods are reviewed in the supplementary.

% % \textbf{Continuous time flows} A separate line of work focuses on building \emph{continuous flows}; in these approaches, the flow's infinitesimal dynamics is parametrized in continuous time, and the corresponding transformation is then found by integrating~\cite{chen2018neural, grathwohl2018ffjord}; Hamiltonian Flows~\cite{rezende2015variational} can also be regarder as such flows.

% % \textbf{Other works} Recently, many works have proposed ways of incorporating convolutional modules in normalizing flows, for example see~\cite{kingma2018glow, hoogeboom2019emerging, karami2019invertible}. In particular, ~\cite{finzi2019invertible} presents a formalization of the problem which has some similarities to ours, while concentrating on convolutional layers instead of fully connected ones.
% % Other work has been dedicated to constructing invertible neural networks, see for example \cite{baird2005one, jacobsen2018revnet, gomez2017reversible}.

% % \begin{itemize}
% %     % \item Reviews: \cite{papamakarios2019normalizing}
% %     % \item NICE \cite{dinh2014nice}
% %     % \item Conditional Density Estimation with Bayesian Normalising Flows (potentially interesting comparison on the Nonstationary ICA since conditional density estimation?) \cite{trippe2018conditional}
% %     % \item Glow \cite{kingma2018glow}
% %     % \item RealNVP \cite{dinh2016density}
% %     % \item Invertible convolutional networks ~\cite{finzi2019invertible}
% %     \item Neural Networks with Cheap Differential Operators ~\cite{chen2019neural}
% % \end{itemize}
